ApacheJIT: A Large Dataset for Just-In-Time Defect Prediction

In this paper, we present ApacheJIT, a large dataset for Just-In-Time defect prediction. ApacheJIT consists of clean and bug-inducing software changes in popular Apache projects. ApacheJIT has a total of 106,674 commits (28,239 bug-inducing and 78,435 clean commits). Having a large number of commits makes ApacheJIT a suitable dataset for machine learning models, especially deep learning models that require large training sets to effectively generalize the patterns present in the historical data to future data.

==> figures/bugs.tex <==
\begin{figure}[h] \centering
 \includegraphics[scale=0.4]{figures/bugs.png}

 \caption{Number of bug-inducing commits in each project}
  \label{fig:bugs}
\end{figure}

% \begin{figure}[h]
% \begin{subfigure}{0.45\textwidth}
%   \includegraphics[scale=0.45]{figures/bugs.png}
%   \caption{Per project} \label{fig:issuesa}
%   \par\medskip % if more vertical separation needed, use \bigskip
%   \includegraphics[scale=0.45]{figures/issues_b.png}
%   \caption{Per year} \label{fig:issuesb}
% \end{subfigure}
% \caption{The number of collected issues per project and per year}\label{fig:issues}
% \end{figure}

==> figures/issues.tex <==
% \begin{figure}[h] \centering
%  \includegraphics[scale=0.4]{figures/issues_a.png}
%  \caption{Distribution of the issues}
%  \label{fig:issues}
% \end{figure}

% \begin{figure}[h]
% \begin{subfigure}{0.45\textwidth}
%   \includegraphics[scale=0.45]{figures/issues_a.png}
%   \caption{Per project} \label{fig:issuesa}
%   \par\medskip % if more vertical separation needed, use \bigskip
%   \includegraphics[scale=0.45]{figures/issues_b.png}
%   \caption{Per year} \label{fig:issuesb}
% \end{subfigure}
% \caption{The number of collected issues per project and per year}\label{fig:issues}
% \end{figure}

\begin{figure}[h] \centering
 \includegraphics[scale=0.45]{figures/issues_a.png}

 \caption{The number of collected issues per project}
  \label{fig:issues}
\end{figure}

==> tables/data.tex <==
\begin{table}[htbp]
\caption{Statistics of ApacheJIT}
\begin{center}
\begin{tabular}{c|c|c|c|c}

\textbf{Set} & \textbf{Bug-inducing} & \textbf{Clean} & \textbf{Total} & \textbf{Bug Ratio} \\
\hline
Training & 22,421 & 22,413 & 44,834 & 0.5000 \\ \hline
Test (Large) & 5,818 & 24,293 & 30,111 & 0.1932 \\ \hline
Test (Small) & 1,448 & 6,078 & 7,526 & 0.1924 \\ \hline
All & 28,239 & 78,435 & 106,674 & 0.2647 \\
\end{tabular}
%   {\raggedright \small * removed after fixing commit collection step (Section \ref{subsec:fixing}) \par}
% \begin{tabular}{|>{\centering\arraybackslash}p{0.09\textwidth}|C{0.09\textwidth}|>{\centering\arraybackslash}p{0.09\textwidth}|>{\centering\arraybackslash}p{0.09\textwidth}|}
% \hline
% {\scriptsize Apache ActiveMQ} & {\scriptsize Apache Camel} & {\scriptsize Apache Cassandra} & {\scriptsize Apache Flink}  \\ \hline
% Apache Groovy & Apache HBase & Apache Hadoop-HDFS & Apache Hive \\ \hline
% \end{tabular}

% \begin{tablenotes}
%     \label{table:pre and post diversity comparison in filtered projects}
%       \small
%       \item ns not significant
%       \item $^*p < 0.1$, $^{**}p < 0.05$
%       \item alternative hypothesis was pre-adoption period diversity is greater
%     \end{tablenotes}
    
    
\label{table:data}
\end{center}
\end{table}



